Hierarchical Planning for Resource Allocation in Emergency Response Systems

A classical problem in city-scale cyber-physical systems (CPS) is resource allocation under uncertainty. Typically, such problems are modeled as Markov (or semi-Markov) decision processes. While online, offline, and decentralized approaches have been applied to such problems, they have difficulty scaling to large decision problems. We present a general approach to hierarchical planning that leverages structure in city-level CPS problems for resource allocation under uncertainty. We use the emergency response as a case study and show how a large resource allocation problem can be split into smaller problems. We then create a principled framework for solving the smaller problems and tackling the interaction between them. Finally, we use real-world data from Nashville, Tennessee, a major metropolitan area in the United States, to validate our approach. Our experiments show that the proposed approach outperforms state-of-the-art approaches used in the field of emergency response.

==> Discussion.tex <==

\section{Discussion}\label{sec:discussion}



==> model.tex <==
\section{Model} \label{sec:model}

We deal with the problem of spatial-temporal resource allocation and response in anticipation of demand for a specific service. We assume that we are given a spatial map
broken up into a finite collection of equally sized cells $G$, and a set of agents $\Lambda$ that need to be allocated in the cells, and subsequently dispatched to the point from where the demand originates. For example, consider the problem of emergency response in urban areas. A set of agents (ambulances in this case) must respond to medical calls across the geographical area. We deal with two specific sub-problems --- 1) stationing, which involves allocating the agents in anticipation of future events, and 2) dispatching, which involves sending a specific agent to the scene of when incidents when they occur. 

While the state space in this resource allocation problem is continuous, it is convenient to view the dynamics as a set of specific decision-making states. As an example, an ambulance moving through an urban area continuously changes the state of the \textit{world}, but presents no scope for decision-making unless an event occurs that needs response. A key component of such problems is that agents need to physically move from their locations to the site of the request in order to accomplish the desired task. This property makes temporal transitions between decision-making states non-memoryless, and is a crucial consideration in designing decision-theoretic models to design optimal response strategies. Specifically, the existence of non-memoryless transitions causes the underlying stochastic process that governs the evolution of the system to be semi-Markovian.

The dynamics of a set of agents working to sequentially make decisions to achieve a common goal can be modeled as a Multi-Agent Semi-Markov Decision Process (MSMDP)\cite{rohanimanesh2003learning}, which can be represented as the tuple $(\Lambda,S,\mathcal{A},P,T,\rho(i,a),\alpha,\mathcal{T})$, where $\Lambda$ is a finite collection of agents and $\lambda_j \in \Lambda$ denotes the $j^{\text{th}}$ agent. The action space of the $j^{\text{th}}$ agent is represented by $A_j$, and $\mathcal{A} = \prod_{i=1}^{m} A_j$ represents the joint action space. We assume that the agents are cooperative and work to maximize the overall utility of the system. The components  $S$, $\rho$ and $P$ are defined as in a standard SMDP. $\mathcal{T}$ represents a termination scheme; note that since agents each take different actions that could take different times to complete, they may not all terminate at the same time. An overview of such schemes can be found in prior literature \cite{rohanimanesh2003learning}. We focus on asynchronous termination, where actions for a particular agent are chosen as and when the agent completes it's last assigned action. 

There are several approaches to solve the MSMDP. One approach is to use a centralized computing mechanism and solve the overall MSMDP directly using dynamic programming~\cite{mukhopadhyayAAMAS18}. The other approach is to use a sampling-based approach that uses a generative model of the world, and weighs potential actions by sampling state-action trajectories ~\cite{MukhopadhyayICCPS}. The canonical approach in this context is to use an appropriately tailored version of the Monte-Carlo Tree Search (MCTS). However, for real-world problems, none of the above approaches scale well to tackle dynamic allocation of resources in urban areas. One way to alleviate the issue of extremely large state spaces and combinatorial action spaces is to use decentralized planning, in which each agent exploits modularity in the planning problem to create a plan for itself\cite{pettet2020algorithmic}. While this approach scales better than centralized planners in solving the problem of dynamic allocation, it is not fast enough to be deployed to the real-world. 

We leverage structure in resource allocation problems to design a hierarchical planning approach that scales significantly better than prior approaches. The key idea in our approach comes from the concept of \textit{macros} in decision-theoretic systems, which denote sub-policies or constrained policies applicable in certain pre-specified regions of the state space~\cite{hauskrecht2013hierarchical}. Our idea is also motivated by the concept of \textit{jurisdictions} or \textit{action-areas} used in public policy, which creates different zones (typically spatial) to segregate and better manage infrastructure. We focus on designing a principled algorithmic approach for identifying region-based segregation of the spatial area under consideration, and create smaller MSMDP problems for each region. While this ensures scalability, it naturally results in performance loss, as agents constrained in one region might be needed in the other region. To tackle this, we create a hierarchical planning approach where the top-level planner, called the inter-region planner, identifies and detects states where ``interaction'' between regions is necessary and finds actions such that the overall utility of the system can be maximized. The low-level planner, called the intra-region planner, works to tackle the problem of allocation and dispatch within a region. The idea of segregating the spatial region under consideration naturally imposes constraints on the overall planning problem. Even though we explicitly account for interactions between the region, it does not guarantee optimality in terms of minimizing the distance traveled by agents (or the time taken by them) to respond to the events. Our goal is to balance the performance of the overall planning approach with scalability by leveraging the correctness of high-level planning with the modularity and efficiency of low-level plans. 

Two key challenges in designing a hierarchical planning approach to tackle the resource allocation problem are as follows: first, we need a principled way of identifying the regions, and second, we need to identify specific states of the world that trigger the high-level planner into action. We describe how we address these challenges below. 

\begin{enumerate}
    \item \textbf{Identifying regions}: We focus on spatially segregating the area under consideration. To achieve this, we use historical data of incident occurrence to partition the set $G$ into clusters using well-known clustering algorithms (the $k$-means algorithm, for example).
    
    \item \textbf{Identifying interactions between regions}: We first introduce the idea of ``global desirability'' in our problem. Consider the case of emergency response by ambulances. It is desirable that all incidents be responded to in a time that is below some pre-specified limit (10 minutes, say). Given a set of $|\Lambda|$ agents, it might be impossible to achieve this goal for an arbitrary demand. The possibility of not achieving such goals makes it impossible to treat them as direct constraints on the system. However, we use such exogenously available goals to guide our hierarchical planning approach. Consider there exists a computationally inexpensive verification/simulation approach $C$ that lets us determine if such goals would be violated given the current configuration of agents $\Lambda$. Then, the planner can automatically check at each decision-making step if such a violation is imminent, and trigger the high-level planner to reconfigure the spatial distribution of agents among the regions. For example, consider that a specific region $r \in R$ experiences a high demand for service. Now consider a point in time when most of the agents allocated to the area are busy. The planner can then identify that in the near future, the region would not be able to meet the global desirability requirements, and seek to re-maneuver agents from some other region to $r$.
    
\end{enumerate}

==> prior_work.tex <==
\section{Prior Work}
\hl{can we rename this section state of the art.}
\begin{figure*}
    \centering
    \includegraphics[height=6cm]{figures/planning_horizon.png}
    \caption{Different approaches to solve a dynamic resource allocation problem under uncertainty. A completely centralized approach (leftmost) deals with a monolithic state representation. Using such a representation, the decision-maker could estimate state transition probabilites using a simulator~\cite{mukhopadhyayAAMAS18} or use an online solution approach~\cite{pettet2020algorithmic}. A completely decentralized approach involves each agent simulating what other agents do and performing its own action estimation (rightmost). Our approach (shown in the middle) segments the original planning problem into multiple sub-problems to improve scalability without agents estimating other agents' actions.}
    \label{fig:planning}
\end{figure*}

A problem modeled as an MDP is typically solved by dynamic programming which assumes availability of the transition dynamics of the system ~\cite{kochenderfer2015decision}. Emergency response has been modeled both by Markovian and semi-Markovian dynamics~\cite{keneally2016markov,mukhopadhyayAAMAS18,pettet2020algorithmic}. Such problems typically evolve in complex urban environments where the transition probabilities are unknown and difficult to estimate in closed-form~\cite{mukhopadhyayAAMAS18}. An approach to tackle the problem is to directly find a policy for the state space by estimating the state transition probabilities while performing canonical policy iteration~\cite{mukhopadhyayAAMAS18}. 
% This poses a problem - the transition functions are unknown, and difficult to model in closed-form. To alleviate this, the Simulate-and-Transform (\textit{SimTrans}) algorithm\cite{mukhopadhyayAAMAS18} uses canonical Policy Iteration with an added computation. In order to estimate values (utilities) of states, the algorithm simulates the entire system of incident occurrence and responder dispatch and keeps track of all states transitions and actions, and gradually builds statistically confident estimates of the transition probabilities.
While such an approach finds a close approximation of the optimal policy (assuming that the estimates of the transition probabilities are close to the true probabilities), this process is extremely slow and unsuited to dynamic environments. As an example, even if a single agent (ambulance in this case) breaks down, the entire process of estimating transition probabilities and learning a policy must be repeated. To better react to dynamic environmental conditions, online decision process approaches such as Monte Carlo Tree Search (MCTS) have been explored~\cite{claes2017decentralised,MukhopadhyayICCPS}. MCTS is a class of heuristic-based search algorithms to find the most promising actions for a given state of a decision-making problem. Given an arbitrary state, MCTS repeatedly simulates the system under consideration to build a search tree that keeps track of the actions taken and the rewards received. 

A somewhat orthogonal approach to solve large-scale MDPs is to use hierarchical planning~\cite{hauskrecht2013hierarchical}. Such an approach focuses on learning local policies, known as \textit{macros}, over subsets of the state space. Our approach is motivated by macros. We show how a large MDP pertaining to emergency response can be divided into smaller MDPs by creating spatial clusters within the area under consideration. The smaller MDPs, which are more tractable by construction, can then be solved by conventional approaches. We also show how hierarchical planning can be used to facilitate an exchange of resources between the spatial regions.
\hl{I think it will be better to merge this section with introduction. that way it might flow better. Introduction can be one and half page - thats fine.}
% The search tree is built in a manner that balances exploration (trying new or sub-optimal actions) and exploitation (greedily exploring the best action). As the number of search iterations increases, the search converges to the optimal action. As an anytime algorithm, MCTS is particularly well suited to the dispatch domain since it is trivial to balance the trade-off between computational time and solution quality. Also, given generative models of different components of the world (incident arrival, responder movement), it is easy to simulate the various complex interactions between agents and the environment.  


==> system_model.tex <==


\section{Background}
\begin{figure*}
    \centering
    \includegraphics[height=4cm]{figures/systemModel.png}
    \caption{Overview of the hierarchical planning approach. We first divide the problem into regions which induce smaller sub-problems. The high-level planner optimizes the distribution of agents among the regions periodically. The low-level planner optimizes the distribution of agents within each region and dispatches agents to incidents as they occur.}
    \label{fig:systemModel}
\end{figure*}

% We assume that the planning problem has Markovian state transitions. While such an assumption is largely applicable to a variety of planning problems, spatial-temporal resource allocation problems often involve semi-Markovian dynamics~\cite{mukhopadhyayAAMAS18,mukhopadhyay2020review}. We circumvent the intricacies of such modeling approaches for now. 

% \hl{I dont think this is really system model - lets call this section understanding the problem. Also note there is some repetition in this section and the previous section. That is why perhaps this section is called understanding the problem and the previous one is just merged with introduction. }




\hl{as part of the this section you should also introduce the concept of ERM - what it is - responders - the networking communication between them and the typical process that takes place. Remember its a CPS conference - so the feedback loop has to be shown. Some of the text from survey can fit here.}

\hl{make sure you clearly specify that in the section on understanding the problem that time is continuous}

We show a broad spectrum of approaches to address resource allocation under uncertainty in Fig.~\ref{fig:planning} from the perspective of multi-agent systems. The most direct approach is to represent the problem as a single Markov decision process (MDP), shown in the extreme left in Fig. ~\ref{fig:planning}. Typically, when real-world problems are modeled as MDPs, the state transitions are difficult to estimate in closed-form. The standard approach then is to use a black-box simulator which is relatively simpler to construct. Then, the simulator can be used to estimate the state transition probability distribution~\cite{mukhopadhyayAAMAS18}. Given the transition distribution, an optimal policy (a mapping from states to actions) can be learned using the well-known policy iteration~\cite{kochenderfer2015decision} algorithm. Another approach is to use an online solution approach, where given a specific state, the simulator is used to aid a heuristic search algorithm like Monte-Carlo tree search (MCTS)~\cite{MukhopadhyayICCPS}.

A different approach is to use a completely decentralized methodology, as shown in the extreme right in Fig. ~\ref{fig:planning}. In such an approach, each agent is entrusted to determine its own course of action. As the agents cooperate to achieve a single goal, agents must estimate what other agents will do in the future as they optimize their actions. For example, \citeauthor{claes2017decentralised}~\citep{claes2017decentralised} show how each agent can build its own Monte Carlo search tree to find near-optimal actions given a state of the world. While such approaches are significantly more scalable than their centralized counterparts, the policy is sub-optimal as agents' estimates of other agents' actions can be highly inaccurate. Note that using high-fidelity models for estimating agents' actions limits scalability and therefore decentralized approaches must rely on computationally cheap heuristics in this regard. Decentralized approaches are crucial to effective emergency response in disaster scenarios where communication networks can break down. In such cases, agents must plan for themselves and cooperate to maximize the overall utility of the system. In urban areas though, agents (first responders and ambulances) typically have access to highly reliable networks and communication is not a constraint. Therefore, approaches that ensure scalability but do not fully utilize full observability of the state space during planning are not suitable for emergency response in urban areas, especially when fast and effective response is of the utmost importance.

Our approach in this paper seeks to find middle ground between completely centralized and completely decentralized solution approaches by leveraging structure in the problems. We create a hierarchical approach to solving the resource allocation problem under uncertainty that scales significantly better than prior approaches. The key idea in our approach comes from the concept of \textit{macros} in decision-theoretic systems, which denote sub-policies or constrained policies applicable in certain pre-specified regions of the state space~\cite{hauskrecht2013hierarchical}. Our idea is also motivated by the concept of \textit{jurisdictions} or \textit{action-areas} used in public policy, which creates different zones (typically spatial) to segregate and better manage infrastructure. We focus on designing a principled algorithmic approach for identifying region-based segregation of the spatial area under consideration, and create smaller planning problems for each region. While this ensures scalability, it naturally results in performance loss, as agents constrained in one region might be needed in the other region. To tackle this, we show how hierarchical planning can be used to facilitate transfer of agents across regions. Specifically, the top-level planner, called the inter-region planner, identifies and detects states where ``interaction'' between regions is necessary and finds actions such that the overall utility of the system can be maximized. The low-level planner, called the intra-region planner, works to tackle the problem of allocation and dispatch within a region. We show the overall approach in Fig. \ref{fig:systemModel}. We first divide the spatial area under consideration in to a set of smaller areas. Resource allocation and dispatch in  each of the smaller areas is treated as a separate planning problem. The high level planner optimizes the distribution of agents among the regions based on global constraints and a utility function. The low level planner optimizes the distribution of agents within each region and dispatches agents to incidents as they occur.


